Efficient Cubature Rules

73 new cubature rules are found for three standard multidimensional integrals with spherically symmetric regions and weights, using direct search with a numerical zero-finder. All but four of the new rules have fewer integration points than known rules of the same degree, and twenty are within three points of M{\"o}ller's lower bound. Most have all positive coefficients and most have some symmetry, including some supported by one or two concentric spheres. They include degree 7 formulas for integration over the sphere and Gaussian-weighted integrals over all space, each in 6 and 7 dimensions, with 127 and 183 points, respectively.

==> Makefile <==
figs=pyramids.eps hoops-1-16-10.eps hoops-1-1-7-7-21.eps plot3e2.eps

all: sigma.pdf

sigma.dvi: sigma.tex $(figs) tableE2.tex tableE1.tex tableS.tex
	latexmk sigma

sigma.ps: sigma.dvi
	dvips sigma -Ppdf -o sigma.ps

sigma.pdf: sigma.ps
	ps2pdf $<

clean:
	rm -f *.exact *.ps sigma.dvi sigma.aux sigma.log sigma.fls sigma.blg sigma.spl sigma.bib
distclean: clean
	rm -f sigma.pdf


check:
	@echo "Duplicate entries in double.txt..."
	@grep dimensions double.txt | sort | uniq -d
	@echo "Duplicate entries in quad.txt (expecting 8)..."
	@grep '^# [A-Z].*dimensions' anc/quad.txt | sort | uniq -d
	@echo "Low precision rules in quad.txt..."
	@awk '								\
	    /==>/{f=$$2}						\
	    /dimensions/{p=$$2}						\
	    /err/{							\
	    	err=gensub(/error=/,"",1,$$NF);				\
	    	if (err+0>1E-32) printf("    %s, %s: %g\n",f,p,err);	\
	    	next;}' anc/quad.txt 
	@echo "correct counts of rules in text..."
	@grep "New Cubature Rules for" sigma.tex >tmp # get counts from table captions
	@grep ".. new cubature rules" sigma.tex >>tmp # get total count from abstract
	@wc tab*tex >>tmp                             # count the lines in each table
	@awk '													\
	    /Rules.*r\^2/{numE2=$$2}										\
            /Rules.*n\^r/{numE1=$$2}										\
            /Rules.*S_n/{numS=$$2}										\
            /[0-9][0-9] new cubature rules/{									\
                i=match($$0,/[0-9][0-9] new cubature rules/);							\
                str=substr($$0,i);										\
                claimed=substr(str,1,2);                       }						\
            /tableE2/{if($$1!=numE2)printf("    There are %d new rules for E2 (not %d).\n",$$1,numE2)}		\
            /tableE1/{if($$1!=numE1)printf("    There are %d new rules for E1 (not %d).\n",$$1,numE1)}		\
            /tableS/ {if($$1-1!=numS) printf("    There are %d new rules for S (not %d).\n", $$1-1,numS)}	\
            END {												\
                total=(numE2+numE1+numS);                                                                       \
                if(claimed!=total)printf("    There are %d new rules in all (not %d as in abstract).\n", total, claimed)}' tmp



==> tmp <==
  \caption{ 25 New Cubature Rules for $E_n^{r^2}$.}\label{tab:summaryE2}
  \caption{ 21 New Cubature Rules for $E_n^r$.}\label{tab:summaryE1}
  \caption{ 21 New Cubature Rules for $S_n$.}\label{tab:summaryS}
  67 new cubature rules are found for three standard 
  21  388 2285 tableE1.tex
  25  469 2886 tableE2.tex
  22  414 2472 tableS.tex
  68 1271 7643 total

